Automatic-differentiation-enabled dynamic parameter retrieval with sub-pulse-width resolution

Time-resolved terahertz time-domain spectroscopy (THz-TDS) is a phase-sensitive tool in condensed matter physics for tracking photoinduced non-equilibrium dynamics of low-energy elementary excitations. However, the measured response function, optical conductivity $\sigma(\omega,t_{pp})$, becomes unreliable in reporting the state of matter when material properties drastically change on a timescale comparable to or less than the probe pulse duration, obscuring the sub-pulse-width dynamics. To resolve this issue, we present a full-waveform inversion framework inspired by the multi-dimensional retrieval philosophy of frequency-resolved optical gating (FROG). By leveraging the automatic differentiation (AD) technique and the two-dimensional time-domain signal $E(t_{g},t_{pp})$, we show one can uniquely solve the inverse problem, at the sub-pulse-width resolution, of retrieving physical observables that are still well-defined, i.e., time-dependent scattering rate $\gamma(t)$, plasma frequency $\omega_\mathrm{p}(t)$ and resonance frequency $\omega_0(t)$, while the response functions are not. Further optimization by gradient-based routines (Adam + L-BFGS) via JAX makes the method exceptionally robust against experimental noise and probe pulse distortions. The validity of the AD-enabled methodology is benchmarked both by a self-consistent numerical approach and by experimental data from real ultrafast THz spectroscopy measurements.

==> fig3/fig3_content.tex <==
%% fig3_content.tex — two-column internal layout, scaled to \columnwidth in main doc.
%%
%% Left column:  dg, dwp (Drude, 2 panels), lg, lw0, lwp (Lorentz, 3 panels)
%% Right column: dlgd, dlwpd, dlgl, dlw0, dlwpl (Drude+Lorentz, 5 panels)

%% ── Drude model: upper left (2 parameters) ────────────────────────────────────

\begin{axis}[
    name=dg,
    paperplot, width=8cm, height=3.5cm,
    title={(a) Drude},
    title style={font=\small\bfseries, at={(0.5,1.0)}, anchor=south, yshift=2pt},
    xmin=0, xmax=8, xticklabels={},
    ylabel={$\gamma$ (ps$^{-1}$)},
    yticklabel style={text width=3em, align=right},
    axis background/.style={fill=activeshade},
]
\addplot[truered, dashed, line width=1.8pt, forget plot]
    table[x=time, y=gamma_true]{fig3/data_complex_gamma.dat};
\addplot[recblue, line width=1.5pt, forget plot]
    table[x=time, y=gamma_rec]{fig3/data_complex_gamma.dat};
\end{axis}

\begin{axis}[
    name=dwp,
    at={(dg.south west)}, anchor=north west,
    paperplot, width=8cm, height=3.5cm,
    xmin=0, xmax=8, xlabel={Time (ps)},
    ylabel={$\omega_p$ (rad/s)},
    scaled y ticks=base 10:-14,
    ytick scale label code/.code={},
    yticklabel style={text width=3em, align=right},
    axis background/.style={fill=activeshade},
]
\node[anchor=south west, font=\scriptsize] at (rel axis cs:0,1) {$\times10^{14}$};
\addplot[truered, dashed, line width=1.8pt, forget plot]
    table[x=time, y=wp_true]{fig3/data_complex_wp.dat};
\addplot[recblue, line width=1.5pt, forget plot]
    table[x=time, y=wp_rec]{fig3/data_complex_wp.dat};
\end{axis}

%% ── Lorentz model: lower left (3 parameters) ──────────────────────────────────

\begin{axis}[
    name=lg,
    at={($(dwp.outer south west)+(0,-0.4cm)$)}, anchor=outer north west,
    paperplot, width=8cm, height=3.5cm,
    title={(b) Lorentz},
    title style={font=\small\bfseries, at={(0.5,1.0)}, anchor=south, yshift=2pt},
    xmin=0, xmax=18, xticklabels={},
    ylabel={$\gamma$ (ps$^{-1}$)},
    ymin=0, ymax=8,
    ytick={0,2,4,6,8}, yticklabels={,2,4,6,8},
    yticklabel style={text width=3em, align=right},
]
\fill[activeshade] (axis cs:7,0) rectangle (axis cs:11,8);
\draw[sampleedge, dashed, line width=0.5pt] (axis cs:7,0)--(axis cs:7,8);
\draw[sampleedge, dashed, line width=0.5pt] (axis cs:11,0)--(axis cs:11,8);
\addplot[truered, dashed, line width=1.8pt, forget plot]
    table[x=time, y=gamma_true]{fig3/data_lorentz_gamma.dat};
\addplot[recblue, line width=1.5pt, forget plot]
    table[x=time, y=gamma_rec]{fig3/data_lorentz_gamma.dat};
\end{axis}

\begin{axis}[
    name=lw0,
    at={(lg.south west)}, anchor=north west,
    paperplot, width=8cm, height=3.5cm,
    xmin=0, xmax=18, xticklabels={},
    ylabel={$\omega_0/2\pi$ (THz)},
    ymin=0, ymax=3,
    ytick={0,1,2,3}, yticklabels={,1,2,},
    yticklabel style={text width=3em, align=right},
]
\fill[activeshade] (axis cs:7,0) rectangle (axis cs:11,3);
\draw[sampleedge, dashed, line width=0.5pt] (axis cs:7,0)--(axis cs:7,3);
\draw[sampleedge, dashed, line width=0.5pt] (axis cs:11,0)--(axis cs:11,3);
\addplot[truered, dashed, line width=1.8pt, forget plot]
    table[x=time, y=w0_true]{fig3/data_lorentz_w0.dat};
\addplot[recblue, line width=1.5pt, forget plot]
    table[x=time, y=w0_rec]{fig3/data_lorentz_w0.dat};
\end{axis}

\begin{axis}[
    name=lwp,
    at={(lw0.south west)}, anchor=north west,
    paperplot, width=8cm, height=3.5cm,
    xmin=0, xmax=18, xlabel={Time (ps)},
    ylabel={$\omega_p$ (rad/s)},
    scaled y ticks=base 10:-14,
    ytick scale label code/.code={},
    ytick={0,2e14,4e14,6e14}, yticklabels={{0},{2},{4},{6}},
    yticklabel style={text width=3em, align=right},
]
\node[anchor=south west, font=\scriptsize] at (rel axis cs:0,1) {$\times10^{14}$};
\pgfplotsextra{
    \coordinate (sha) at (axis cs:7,0); \coordinate (shb) at (axis cs:11,0);
    \fill[activeshade] (sha |- current axis.south west) rectangle (shb |- current axis.north east);
    \draw[sampleedge, dashed, line width=0.5pt] (sha |- current axis.south west)--(sha |- current axis.north east);
    \draw[sampleedge, dashed, line width=0.5pt] (shb |- current axis.south west)--(shb |- current axis.north east);
}
\addplot[truered, dashed, line width=1.8pt, forget plot]
    table[x=time, y=wp_true]{fig3/data_lorentz_wp.dat};
\addplot[recblue, line width=1.5pt, forget plot]
    table[x=time, y=wp_rec]{fig3/data_lorentz_wp.dat};
\end{axis}

%% ── Drude + Lorentz model: right column (5 parameters) ───────────────────────

\begin{axis}[
    name=dlgd,
    at={(9.0cm, 1.92cm)}, anchor=north west,
    paperplot, width=8cm, height=3.6cm,
    title={(c) Drude + Lorentz},
    title style={font=\small\bfseries, at={(0.5,1.0)}, anchor=south, yshift=2pt},
    xmin=0, xmax=12, xticklabels={},
    ylabel={$\gamma_D$ (ps$^{-1}$)},
    ymin=0, ymax=7,
    ytick={0,2,4,6}, yticklabels={,2,4,6},
]
\pgfplotsextra{
    \coordinate (csha) at (axis cs:2,0); \coordinate (cshb) at (axis cs:10,0);
}
\addplot[truered, dashed, line width=1.8pt, forget plot]
    table[x=time, y=gamma_D_true]{fig3/case1_gamma_D.dat};
\addplot[recblue, line width=1.5pt, forget plot]
    table[x=time, y=gamma_D_rec]{fig3/case1_gamma_D.dat};
\end{axis}

\begin{axis}[
    name=dlwpd,
    at={(dlgd.south west)}, anchor=north west,
    paperplot, width=8cm, height=3.6cm,
    xmin=0, xmax=12, xticklabels={},
    ylabel={$\omega_{p,D}$ (rad/s)},
    scaled y ticks=base 10:-14,
    ytick scale label code/.code={},
    ymin=2e14, ymax=6e14,
    ytick={2e14,3e14,4e14,5e14,6e14}, yticklabels={{},{3},{4},{5},{}},
]
\node[anchor=south west, font=\scriptsize] at (rel axis cs:0,1) {$\times10^{14}$};
\addplot[truered, dashed, line width=1.8pt, forget plot]
    table[x=time, y=wp_D_true]{fig3/case1_wp_D.dat};
\addplot[recblue, line width=1.5pt, forget plot]
    table[x=time, y=wp_D_rec]{fig3/case1_wp_D.dat};
\end{axis}

\begin{axis}[
    name=dlgl,
    at={(dlwpd.south west)}, anchor=north west,
    paperplot, width=8cm, height=3.6cm,
    xmin=0, xmax=12, xticklabels={},
    ylabel={$\gamma_L$ (ps$^{-1}$)},
    ymin=0, ymax=3.5,
    ytick={0,1,2,3,3.5}, yticklabels={,1,2,3,},
]
\addplot[truered, dashed, line width=1.8pt, forget plot]
    table[x=time, y=gamma_L_true]{fig3/case1_gamma_L.dat};
\addplot[recblue, line width=1.5pt, forget plot]
    table[x=time, y=gamma_L_rec]{fig3/case1_gamma_L.dat};
\end{axis}

\begin{axis}[
    name=dlw0,
    at={(dlgl.south west)}, anchor=north west,
    paperplot, width=8cm, height=3.6cm,
    xmin=0, xmax=12, xticklabels={},
    ylabel={$\omega_0/2\pi$ (THz)},
    ymin=1.35, ymax=3.05,
    ytick={1.6,2.0,2.4,2.8}, yticklabels={1.6,2.0,2.4,2.8},
]
\addplot[truered, dashed, line width=1.8pt, forget plot]
    table[x=time, y expr=\thisrow{omega_0_true}/6.2832e12]{fig3/case1_omega_0.dat};
\addplot[recblue, line width=1.5pt, forget plot]
    table[x=time, y expr=\thisrow{omega_0_rec}/6.2832e12]{fig3/case1_omega_0.dat};
\end{axis}

\begin{axis}[
    name=dlwpl,
    at={(dlw0.south west)}, anchor=north west,
    paperplot, width=8cm, height=3.6cm,
    xmin=0, xmax=12, xlabel={Time (ps)},
    ylabel={$\omega_{p,L}$ (rad/s)},
    scaled y ticks=base 10:-14,
    ytick scale label code/.code={},
    ymin=0.8e14, ymax=3.8e14,
    ytick={1e14,2e14,3e14}, yticklabels={{1},{2},{3}},
]
\node[anchor=south west, font=\scriptsize] at (rel axis cs:0,1) {$\times10^{14}$};
\addplot[truered, dashed, line width=1.8pt, forget plot]
    table[x=time, y=wp_L_true]{fig3/case1_wp_L.dat};
\addplot[recblue, line width=1.5pt, forget plot]
    table[x=time, y=wp_L_rec]{fig3/case1_wp_L.dat};
\end{axis}

%% Unified green fill for panel (c) on the background layer, then dashed borders on top
\begin{pgfonlayer}{background}
    \fill[activeshade] (csha |- dlgd.north) rectangle (cshb |- dlwpl.south);
\end{pgfonlayer}
\draw[sampleedge, dashed, line width=0.5pt] (csha |- dlgd.north) -- (csha |- dlwpl.south);
\draw[sampleedge, dashed, line width=0.5pt] (cshb |- dlgd.north) -- (cshb |- dlwpl.south);

%% ── Separator lines ──────────────────────────────────────────────────────────
\draw[black, line width=1.2pt] (dg.south west)  -- (dg.south east);
\draw[black, line width=1.2pt] (lg.south west)  -- (lg.south east);
\draw[black, line width=1.2pt] (lw0.south west) -- (lw0.south east);
\draw[black, line width=1.2pt] (dlgd.south west)  -- (dlgd.south east);
\draw[black, line width=1.2pt] (dlwpd.south west) -- (dlwpd.south east);
\draw[black, line width=1.2pt] (dlgl.south west)  -- (dlgl.south east);
\draw[black, line width=1.2pt] (dlw0.south west)  -- (dlw0.south east);

%% ── Legend below panel (c) ──────────────────────────────────────────────────
\coordinate (legmid) at ($(dlwpl.outer south west)!0.5!(dlwpl.outer south east)+(0,-0.4cm)$);
\draw[truered, dashed, line width=1.8pt]
    ($(legmid)+(-1.8cm,0)$) -- ($(legmid)+(-1.1cm,0)$);
\node[anchor=west, font=\small] at ($(legmid)+(-1.0cm,0)$) {True};
\draw[recblue, line width=1.5pt]
    ($(legmid)+(0.0cm,0)$) -- ($(legmid)+(0.7cm,0)$);
\node[anchor=west, font=\small] at ($(legmid)+(0.8cm,0)$) {Reconstructed};

